Visual Exploration of Machine Learning Model Behavior with Hierarchical Surrogate Rule Sets

One of the potential solutions for model interpretation is to train a surrogate model: a more transparent model that approximates the behavior of the model to be explained. Typically, classification rules or decision trees are used due to the intelligibility of their logic-based expressions. However, decision trees can grow too deep and rule sets can become too large to approximate a complex model. Unlike paths on a decision tree that must share ancestor nodes (conditions), rules are more flexible. However, the unstructured visual representation of rules makes it hard to make inferences across rules. To address these issues, we present a workflow that includes novel algorithmic and interactive solutions. First, we present Hierarchical Surrogate Rules (HSR), an algorithm that generates hierarchical rules based on user-defined parameters. We also contribute SuRE, a visual analytics (VA) system that integrates HSR and interactive surrogate rule visualizations. Particularly, we present a novel feature-aligned tree to overcome the shortcomings of existing rule visualizations. We evaluate the algorithm in terms of parameter sensitivity, time performance, and comparison with surrogate decision trees and find that it scales reasonably well and outperforms decision trees in many respects. We also evaluate the visualization and the VA system by a usability study with 24 volunteers and an observational study with 7 domain experts. Our investigation shows that the participants can use feature-aligned trees to perform non-trivial tasks with very high accuracy. We also discuss many interesting observations that can be useful for future research on designing effective rule-based VA systems.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/01-old_intro.tex <==
In this work, we introduce SuRE, a pipeline of generating and visualizing surrogate \textit{If-then} rules to explain the behaviors of a Machine Learning (ML) model. \textit{If-then} rules are widely used in our daily lives for decision making, for example, \textit{``If the weather is good, then I will go grocery.''}. As such, for people without a technical background, a statement in an \textit{if-then} format is intuitive and straightforward as a way of explaining how an ML model makes decisions on a single instance or a group of instances. 

Explaining model behaviors remains to be an important topic across AI and VIS communities. Researchers have extracted tree structures to explain a trained neural network~\cite{craven1996extracting} decades ago. With the development of AI and the increasing complexity of high-performed models, the explanation of model behaviors becomes crucial. It helps humans validate and improve a model, make more informed decisions and gain more trust while using a model~\cite{hong2020human}. In recent years, there is a resurgence of algorithms for model explanation ~\cite{lakkaraju2016interpretable,lundberg2017unified,ribeiro2016should,wang2017bayesian}. Many visual analytics systems~\cite{} are also introduced to assist model developers and domain experts to understand, analyze and debug a trained ML model. 

In general, the explanations of an ML model can be obtained from the model itself if it is interpretable and transparent enough, or from a post-hoc process without exposing the internal structure of a trained model. Linear models and decision tree are commonly used as interpretable models~\cite{molnar2019}. For more complex models such as Deep Neural Network (DNN) and ensemble models, it is hard to interpret their internal logic directly, especially for humans without a strong technical background such as domain experts and end-users. As such, post-hoc explanations are necessary to explain what a model has learnt and how the model makes decisions. In practice, domain experts and regulators often need to gain an overview of the model and also to focus on specific areas of the decision space. For this reason, we focus on the post-hoc methods of explaining the model behaviors in specific regions of interest, also known as ``global'' methods, instead of those explaining a single decision made by a model. 

In general, post-hoc global methods adopt different ``lenses'' to inspect model behavior. We can roughly organize them into two major approaches: those with a \textit{focus on features} and those with a \textit{focus on instances}. Methods that focus on features, describe model behavior in terms of the role individual or groups of features play in the model. These methods typically reveal model behavior either by computing various forms of feature relevance (for the whole model or for sub-groups)~\cite{fisher2018model, lundberg2017unified} or by extracting from the model information about how prediction scores vary in relation to changes in the values of one or two features of interest~\cite{friedman2001greedy, apley2016visualizing} (often visualized with line charts or heat maps).

Methods that focus on instances, describe model behavior in terms of data properties. In this space the most common approach is to use logic-based surrogate models: transparent models trained using the output of the original model as training data with the intent of simulating its behavior. Typically these models are trained using either rule-based learning or decision trees~\cite{quinlan1986induction,quinlan2014c4} and they generate full descriptions of model behavior through sets of logic-based structures and statements. Although model explanations that focus on features are useful when inspecting how feature(s) influence model decisions, they remain to be statistical summaries of features. Surrogate rules, instead, are more descriptive because an \textit{if-then} statement describes how model makes consistent decisions in a specific region. And such statements are straightforward even for people who are not familiar with machine learning. 

To add: limitation and usefulness of decision tree....

% However, there are some limitations when using surrogate trees or rules to interpret and analyze model behavior. The first is the limitation of a single tree-structure. On a single decision tree, all the rules (decision paths) have common ancestors and all the paths are disjoint. 

% Contribution:
% \begin{itemize}
%     \item a pipeline for visual analytics of surrogate rules
%     \item a novel visual design for hierarchical inspection of surrogate rules
%     \item a user study of how people interact with the proposed pipeline SuRE as well as how hierarchical logic visualization can help with model understanding
% \end{itemize}

Storyline:
1. There are many problems of using rules to explain and understand a machine learning model\\
	1) the trade-off between complexity and fidelity\\
	2) recent work on rule visualization treat all the conditions in a rule equally which leads to some problem because many rules contain a hierarchical structure during rule generation. \\

2. Hierarchical structure is important to be shown to users for two reasons:

    1) the rules are hierarchical, if we use the tree structure directly, there are some rules not useful, and there are a lot of redundancy and is not space effective\\
	2) humans can prune the rules by themselves by looking at the visualization \\
	3) in our collaboration with some chemists, they explicitly say that they want to check how the subpopulation narrow down\\

3. So we want to design a pipeline that integrates complexity/fidelity control by humans, as well as the rule visualization that assist users to inspect hierarchical structure of rules.

4.  Our contribution includes:
\begin{itemize}
    \item  a human-in-the-loop pipeline of rule generation and rule exploration
	\item   visual designs for rule logic that reveals the hierarchical structure of rules
	\item   a readability study that evaluates the proposed new design
	\item   an interview in which we collect information about how domain experts use rules and some feedback on the proposed pipeline and visualizations.
\end{itemize}


==> sections/07-old_user_study.tex <==
\section{Evaluation}
We evaluated the usability and usefulness of the pipeline of SuRE in multiple ways following the guidance from visualization community~\cite{isenberg2013systematic,lam2011seven}. First, we present an online usability test with 24 participants in which we evaluated whether humans can read and extract information from the novel lattice design of rule logic correctly. Then we report the feedback on SuRE collected through in-depth interviews with 7 domain experts. 

For both evaluation, we used the PIMA diabetes dataset~\cite{smith1988using} to generate rule sets and the corresponding visualization as an example to introduce necessary concepts related to rules, ML models and visualizations. As for the actual studies, we apply the proposed pipeline to a loan application dataset~\cite{fico} that is more challenging, leading to more complex rule sets and visual representations. More detailed description for the study procedures is included in the following subsections.

% \subsection{Usability Study}
\subsection{Evaluation of the Lattice Design}
The goal of this study is to test whether users can accurately extract and search for information from the proposed lattice-like visual design of rules. To this purpose, we conducted usability tests with 24 students from Computer Science department focusing only on the lattice design.

\textbf{Tasks.} We designed two types of tasks which simulate how humans extract information from a rule set to understand model behavior. Imagine that a doctor is inspecting the rule set that describes disease diagnosis process, he or she can (1) read through the present rules and validate the disease diagnosis logic; or (2) has some hypotheses in mind or is highly interested in specific features or classes, and needs to seek for relevant information for further analysis. As such, we formalize the following tasks: 

\begin{itemize}
    \item[\textbf{T1}] Read information from the presented visualization.
    
    \item[\textbf{T2}] Look for visual element(s) that contain desired properties.
\end{itemize}

\begin{figure}
 \centering 
 \includegraphics[width=\columnwidth]{pic/usability_t1.png}
%  \vspace*{-.6cm}
 \caption{The screenshot of the actual test in usability study for task T1.}
%  \vspace*{-.7cm}
 \label{fig:usability_t1}
\end{figure}

\begin{table*}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{T1} & \multicolumn{6}{c|}{T2} \\\hline
      Q1 & Q2 & Q3 & Q4 & Q5 & Q6 & Q7 & Q8 & Q9 & Q10 \\\hline
      24/24 & \textbf{23}/24 & \textbf{23}/24 & \textbf{23}/24 & 24/24 & 24/24 & 24/24 & 24/24 & \textbf{23}/24 & \textbf{23}/24 \\ 
    \hline
    \end{tabular}
    \caption{The performance of each question. The first number in each cell represents the number of people that answered this question correctly, while the second value 24 is the total number of participant. For all the questions, most people can answer them correctly.}
    \label{tab:usability_test}
\end{table*}

For the first type of task (T1), we presented a static lattice representation of rules to participants and then ask them what \textit{feature name}, \textit{condition}, \textit{error rate}, or \textit{support} a specific node shows (Fig.~\ref{fig:usability_t1}). For the second type of task (T2), we approximate the case where humans have a question or hypothesis in mind, and he or she needs to find out the answer from the rule set. So we ask the participants to click a node in the presented visualization that matches the given description. For example, one of the questions we asked is "Please select the node that covers the least of people." All the questions we asked in the actual test are included in the Appendix~\ref{append:test_question}.

\textbf{Task Performance Measurements.} Because our goal in this study is to test whether humans can extract information correctly, accuracy is used as the main measurement. For T2, there may be more than one node that matches the given description. We asked the participants only need to choose one answer. As for the result analysis, the first question of each task type was used only for habituation to the task and was eliminated from the analysis. 

We also asked the participants to report their subjective sense of effort for each task. This score is measured at the end of each task by answering the question of ``To what extent do you agree with the following statement: \textit{It was easy for me to answer the questions.}''

\textbf{Participants.} A total of 24 volunteers were recruited to participate to the study. We first sent an email to all the students in the Computer Science and Engineering department at the NYU School of Engineering and asked students who were interested in this study to fill a form. Then we contacted these students and scheduled the studies with them.

\textbf{Procedure.} We organized 4 online meetings via Zoom. In each meeting, there are 3 to 9 participants and we encouraged them to ask any questions they have when we introduce the visualization and the tasks. In the beginning of each study, we collected the consent form from each participant. And then we introduced how to read the lattice visualization and what tasks we are going to ask them to perform. In the task introduction part, we also asked the participants to answer a few questions in the quiz (embedded in Zoom) to validate whether they understand the concepts and are ready for the test. In the end, we asked the participants to finish the actual test via Qualtrics. They were required to mute themselves during the test and were allowed to direct message the authors for any questions related to the test.

\textbf{Results.} For both task 1 and task 2, most people can answer all the questions correctly. As shown in Table ~\ref{tab:usability_test}, on only five questions (Q2, Q3, Q4, Q9 and Q10) that do not have a $100\%$ accuracy. Even though, an accuracy of $95.8\%$ (23/24) is quite high considering that these participants are introduced to this visualization for the first time. 

As for the subjective sense of effort, most participants agreed that the two tasks are easy for them ($95.8\%$ for Task 1 and $91.7\%$ for Task 2, see  Fig.~\ref{fig:usability_easy}). For Task 1, $87.5\%$ of participants extremely agreed that this task was easy to answer. However, only $37.5\%$ of participants extremely agreed that task 2 was easy to answer. This makes sense because task 2 not only requires participants to read the information from the visualization but also to compare and search desired visual elements in the view. We also noticed that no one thought the questions for both task 1 and task 2e were not easy given this new visualization. It is a good signal that learning such a lattice-like visualization of hierarchical rule logic information is easy for most people. Therefore, we believe that humans are able to correctly and easily extract information from the proposed lattice visualization of rules.


\begin{figure}
 \centering 
 \includegraphics[width=\columnwidth]{pic/usability_easy.png}
%  \vspace*{-.6cm}
 \caption{The proportion of responses to the question of ``To what extent do you agree with the following statement''.}
%  \vspace*{-.7cm}
 \label{fig:usability_easy}
\end{figure}

\subsection{Interviews with Domain Experts} 
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
         Interviewee & Degree & Experience Level & Role \\\hline
         P1 &  Master & entry-level & Data Scientist \\\hline
         P2 & Bachelor & entry-level & Software Engineer \\\hline
         P3 & PhD & entry-level & Research Scientist \\\hline
         P4 & PhD & senior & Research Scientist \\\hline
         P5 & PhD & senior & Research Scientist \\\hline
         P6 & PhD & junior & Data Scientist \\\hline
         P7 & Master & junior & Data Scientist \\\hline
    \end{tabular}
    \caption{We conducted in-depth interviews with domain experts from a financial company. Among all the interviewees, only P2 is a software engineer and was working on the development of an ML platform. The rest of the interviewees are data scientists and researchers who work a lot on model development and data analysis.}
    \label{table:interviewee}
\end{table}

\begin{table*}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        \textbf{Pattern} & \textbf{Mode} & \textbf{Question Category} & \textbf{Example Question}\\\hline
       \multirow{6}{*}{Exploratory}  & \multirow{2}{*}{Querying} & Node with Property &``Which node covers the most instances?'' \\
        & & Rule Set with Property & ``What is the rule set with fewer rules/shorter rules like?'' \\\cline{2-4}
       
        & Learning & Feature Familiarization* & ``What is the distribution of the features?'', ``Is the feature monotonic?'' \\\cline{2-4}
        
        & \multirow{2}{*}{Comparing} & Node Comparison & ``What are the rules that contain only one condition and high-fidelity enough?''\\
        & & Subgroup Comparison & ``Do two subgroups contain the same group of people?'' \\\cline{2-4}
        
        & Summarizing & Summarization & n/a (write down the insights) \\\hline
        
         \multirow{6}{*}{Confirmatory} & \multirow{3}{*}{Validating} & Validation & ``Does the number of rules for each class match the class distribution?''\\
         & & Feature-error relation & ``whether the usage of a feature increases or decreases errors?'' \\
         & & Feature Interaction & ``How does this feature influence the prediction distribution given a condition?'' \\\cline{2-4}
         
         & \multirow{3}{*}{Hypothesis Testing} & Hypothesis Testing & ``Is there any subgroup with good bills paid on time predicted as default?'' \\
         & & Threshold Adjustment* & ``What is the prediction distribution for this feature in a narrower range?'' \\
         & & Customized Subgroup* & ``What is model behavior on a subgroup when a condition is added?'' \\
    \hline
    \end{tabular}
    \caption{The questions that people want to answer when using the prototype of SuRE. We categorized these questions or actions into two patterns of six different modes. The question categories with with a star symbol (*) are not explicitly supported in the prototype but are important to some domain experts.}
    \label{table:pattern}
\end{table*}

To evaluate the usefulness of the proposed pipeline and to collect feedback of different visualizations with hierarchical rule logic information, we conducted in-depth expert interviews with 7 domain experts. In this section, we describe the procedure for each interview, the major patterns of using SuRE in a practical setting, as well as other findings and trends we identified through the interviews.

\subsubsection{Study Set-up}
\textbf{Participants.} We invited seven practitioners from a financial company. As shown in Table~\ref{table:interviewee}, our participants have quite different experiences in industry, including people who just started their career (P1, P2, P3) and those who worked with data for more than 10 years (P4, P5). All of these participants have a strong background of machine learning and have had quite different goals working with data and machine learning models. For example, for P1 and P7, their work is more about data analysis and need to extract insights from existing data; while P3 and P5 applied explainable AI (xAI) techniques to assist other departments.

\textbf{Procedure.} We begin each interview with an introduction, during which we clarified the goals of our study, explained three different hierarchical rule logic designs, and provided a brief tutorial regarding the use of our system. Similar to what we have done in the usability test, we set up a simple quiz to check whether the interviewee knows how to read the visualization properly. Then, the experts were allowed to explore the prototype freely using the example visualizations of diabetes data. To make sure the expert is able to interact with the prototype properly, we asked the expert to answer two open-ended questions: (1) \textit{``What is the most probable outcome when ...?''} and (2) \textit{``Given a person is predicted as having diabetes, what characteristics may this person have?''} We then asked the experts to explore and understand a pre-trained model of loan applications~\cite{fico} using the prototype system. In this stage, the interviewees need to follow a "think-aloud" protocol~\cite{fonteyn1993description}, which means they are required to tell us what questions they want to answer and whether they find the answer, or whether there is anything confusing. In the end, we conducted a semi-structured interview which incorporated several questions about visual designs, overall usefulness, general pros and cons of the prototype system as well as how they can imagine such pipeline to be applied with their own data or work. Each interview lasted around 1.5 to 2 hours via Zoom, during which notes were taken and the entire procedure was recorded.

\subsubsection{Lessons Learned}
Through the interviews, we have gained a better understanding of how SuRE can help with model understanding and data analysis, which leads to the following lessons learned:

\textbf{Lesson 1: Patterns of Using Sure.} By observing how the experts used SuRE to understand and analyze model behavior, we identified two different patterns. The first is an \textit{Exploratory} pattern, in which the users get them familiar with the data, the model, or the tool itself. The second is a \textit{Confirmatory} pattern, in which the users have already gained some knowledge from the first pattern and need to validate the knowledge or test some hypotheses. If the expert have already known the data and related business well, they may turn into a Confirmatory pattern and focus on the features of interest directly.

We further analyzed the questions that people want to answer when using the prototype of SuRE into the two patterns and categorized them into six different modes. Example questions are listed in the Table~\ref{table:pattern}.

We also noticed that the order of patterns people use to explore the rules and model are quite different in terms of different familiarity levels about the data. For example, P2, who did have too much knowledge about the loan data before the interview, used SuRE mostly to explore the model behavior and then write down his findings as summaries. Different from him, P5 and P7 are experienced data scientists and they already some hypotheses or features of interest before rule exploration. So they use SuRE mostly for validation and hypothesis testing. 

\textbf{Lesson 2: Visual Representations Are Complementary.}
During the rule exploration, we found that people tended to switch between three different visual representations. The experts told us the three views can support the learning and analysis of rules from different aspects and are good at different analysis tasks.

\textit{Text List} is good at comparing the prediction distribution of different rules/subgroups. And it is straightforward for people to know how many rules are involved.

\textit{Hierarchical List} can clearly show the discriminative conditions (condition content) at the top level and it is useful to look at a group of rules or conditions with the same leading condition. Also, it enables comparison of children conditions/nodes of the same parent condition/node.

\textit{Lattice}, however, is really good at indexing the rules contain different values of a features or any feature of interest because of the feature alignment. It is also useful to find out the features that are used frequently after feature ordering. Similar to hierarchical list, a lattice view also enables comparison of children conditions/nodes of the same parent condition/node. Moreover, it is easier to see the prediction changes along a decision path. The squared node design is good at comparing subgroup-level model errors.

\textbf{Lesson 3: Short Descriptions Are Preferred.} People usually focus on one feature (condition) for analysis first. They start from a node at the first layer that is either large enough or pure enough or both. And then they inspect the second conditions or nodes that are linked with a condition of interest at the first layer. They rarely ask how three features interact with each other. Even if they inspect rules with more than 2 conditions, they reason about the feature values individually.

\textbf{Lesson 4: Understand Data But Not Model.} SuRE helps validate the model behavior and also help people to learn more about the data by understanding what the model learns. P6 said, ``It's either that the model is wrong or I don't understand the problem well enough''. Another participant, P5, also told us that he found rules are really useful here and want to directly apply rules as a white-box model to analyze and understand his own data.






